Multi-Model Learning for Real-Time Automotive Semantic Foggy Scene Understanding via Domain Adaptation

Robust semantic scene segmentation for automotive applications is a challenging problem in two key aspects: (1) labelling every individual scene pixel and (2) performing this task under unstable weather and illumination changes (e.g., foggy weather), which results in poor outdoor scene visibility. Such visibility limitations lead to non-optimal performance of generalised deep convolutional neural network-based semantic scene segmentation. In this paper, we propose an efficient end-to-end automotive semantic scene understanding approach that is robust to foggy weather conditions. As an end-to-end pipeline, our proposed approach provides: (1) the transformation of imagery from foggy to clear weather conditions using a domain transfer approach (correcting for poor visibility) and (2) semantically segmenting the scene using a competitive encoder-decoder architecture with low computational complexity (enabling real-time performance). Our approach incorporates RGB colour, depth and luminance images via distinct encoders with dense connectivity and features fusion to effectively exploit information from different inputs, which contributes to an optimal feature representation within the overall model. Using this architectural formulation with dense skip connections, our model achieves comparable performance to contemporary approaches at a fraction of the overall model complexity.

==> tex/8.end-matter.tex <==
%\begin{multicols}{0}
\noindent{\large \textbf{Response to the comments of ICPR 2020
		submission \emph{1315}}} 




%%\title{Multi-Model Learning for Real-Time Automotive Semantic Foggy Scene Understanding \\via Domain Adaptation}
%%

\thispagestyle{empty}

\subsection*{\normalsize \bf  General Remarks}
\noindent First we would thank the reviewers for the valuable feedback and suggestion. As a clarification of our novel contributions, an end-to-end automotive semantic segmentation approach has been proposed which performs: 

\begin{enumerate}
	%\baselineskip=12pt
	\item [(1)] the transformation of imagery from foggy to clear weather conditions.  
	\item [(2)] pixel-wise labelling via a competitive lightweight architecture enabling real-time performance. 
\end{enumerate} 

\noindent Regardless achieving minor improvement in accuracy, most prior work reuse complex networks, making them unable for real-time performance. \\

\noindent In the following, we respond to the specific points from each reviewer in the following: 

\subsection*{\normalsize \bf  Response to Reviewer \#1}
\vspace{-1mm}
\begin{enumerate}[nolistsep] %[topsep=\parskip] %a single \acrshort{rgb}	 	
	{\color{red}\item\noindent The reference to off-the-shelf segmentation networks} is for open-source deep-learning-based methods (we will replace it with \underline{\textbf{established approaches}}). As most of the comparative studies \cite{foggy_pure, foggy18, foggy_old} included in the paper used such existing networks and we compared against them in Table I, we propose a competitive model combines reasonable performance with less resource consumption.
	
	{\color{red}\item\noindent The grammatical error in the sentence `` ...We focus on recent ..''} has been \underline{\textbf{corrected}}.
	
	{\color{red}\item\noindent Missing comparison to other relevant methods on the Supplementary material}: We agree with the reviewer's suggestion, so a table showing the result of comparing our approach against relevant methods is \underline{\textbf{added}}.
\end{enumerate}   

\subsection*{\normalsize \bf  Response to Reviewer \#2}
\vspace{-1mm}
\begin{enumerate}[nolistsep]
	{\color{red}\item\noindent mIoU is worse compare with e.g. Foggy Zurich}:
	As all comparators rely on complex existing segmentation networks which had been criticized \cite{ldfnet} for sacrificing real-time performance at the expense of segmentation accuracy. Moreover, Hanner \textit{et al.} \cite{foggy_pure} fine-tuned their model (as an extra step) on Foggy Synscapes \cite{foggy_pure} (privately large dataset inludes 24500 training images), hence, why they achieved high accuracy. On the other hand, our approach provides a complete solution to deal with complex and effective scene  segmentation  processes  in  an  end-to-end pipeline, designed with a lightweight architecture and allowing real-time performance. 
	
	{\color{red}\item\noindent Comparison over Foggy Cityscapes}:
	We conduct an ablation study in Table II and Figure 7 showing the performance of our proposed method with and without domain adaptation over the Foggy Cityscapes dataset. In contrast, comparative approaches (prior work of \cite{dai2019curriculum, foggy_pure, foggy18, foggy_old}) do not provide any qualitative and quantitative results over Foggy Cityscapes, which means our proposed approach provides additional evaluation.
	
	{\color{red}\item\noindent Typos, errors and general suggestion}:
	All minor typos, errors and general suggestions in the six points the reviewer refers to have been \underline{\textbf{corrected}}.
	
	{\color{red}\item\noindent Enhancing images in the demo}: 
	We agree that the images in the provided demo/video are not very clear as we reduced the size of them. As the reviewer suggests, the images in the demo now are \underline{\textbf{enhanced}}.
\end{enumerate} 

\subsection*{\normalsize \bf  Response to Reviewer \#3}

\begin{enumerate}[nolistsep]
	{\color{red}\item\noindent The contributions of the paper are not entirely clearly stated}: Our proposed approach provides the following: (i) pre-mapping degraded visibility in \textit{foggy} weather conditions to normal by using CycleGAN \cite{CycleGAN2017} and (ii) performing semantic segmentation based on the outputs from the step (i). As an end-to-end pipeline,  our model combines lightweight design  and comparable performance.
	
	{\color{red}\item\noindent Promising results when compared with state-of-the-art} As seen in Table I, our approach performs better than the current state-of-the-art \cite{foggy_pure} and remains competitive with \cite{dai2019curriculum, foggy_pure, foggy18, foggy_old}. Most importantly,  our proposed approach achieves comparable performance with a lightweight, computationally superior pipeline design. We have specifically \underline{\textbf{improved}} the presentation of this information in the paper.
	
	{\color{red}\item\noindent Comparisons to the state-of-the-art is not promising}: Our model is distinguished by all competing models by providing real-time performance with less computational resources. In addition, our method outperforms the state-of-the-art segmentation approaches \cite{bisenet} on the benchmark datasets \cite{foggy19, foggy18}.
	
	{\color{red}\item\noindent Low computational complexity and real-time performance with fully convincing matter}: We propose an end-to-end network architecture with the challenge of tackling adverse weather and semantic segmentation. In Table I, some available results on the computational complexity of existing approaches are compared with our proposed approach and show that our approach offers a better balance between robustness and real-time operation.
\end{enumerate}



